Laconic: Streamlined Load Balancers for SmartNICs

Load balancers are pervasively used inside today's clouds to scalably distribute network requests across data center servers. Given the extensive use of load balancers and their associated operating costs, several efforts have focused on improving their efficiency by implementing Layer-4 load-balancing logic within the kernel or using hardware acceleration. This work explores whether the more complex and connection-oriented Layer-7 load-balancing capability can also benefit from hardware acceleration. In particular, we target the offloading of load-balancing capability onto programmable SmartNICs. We fully leverage the cost and energy efficiency of SmartNICs using three key ideas. First, we argue that a full and complex TCP/IP stack is not required for Layer-7 load balancers and instead propose a lightweight forwarding agent on the SmartNIC. Second, we develop connection management data structures with a high degree of concurrency with minimal synchronization when executed on multi-core SmartNICs. Finally, we describe how the load-balancing logic could be accelerated using custom packet-processing accelerators on SmartNICs. We prototype Laconic on two types of SmartNIC hardware, achieving over 150 Gbps throughput using all cores on BlueField-2, while a single SmartNIC core achieves 8.7x higher throughput and comparable latency to Nginx on a single x86 core.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> sections/eval.tex <==
\section{Evaluation}
\label{sec:eval}
We implement our design on both on-path and off-path SmartNICs with \texttt{DPDK 21.11}. We implement \sys in 6k lines of C++ code. In this section, we will first show our testbed setup and compare our system with a state-of-the-art commodity L7 load balancer on synthetic benchmarks. We then evaluate \sys on a realistic workload. This work does not involve any ethical issues. 
\subsection{Experiment Setup}
Our testbed consists of 5 x86 servers with Intel Xeon 5218 CPU and 64GB of memory. Each server is equipped with a Mellanox ConnectX 5 two-port NIC. The link speed of each individual port is 100Gbps. We use a dedicated set of servers to deploy SmartNICs. The on-path SmartNIC we use is a Marvell LiquidIO 3 CN3380 with 2x50Gbps ports. The off-path SmartNIC used in our deployment is a Mellanox BlueField-2 MBF2H516C-CECOT with 2x100Gbps ports.

An Arista DCS-7060CX switch is configured with VLAN and L4-routing and partitions the clients and servers into two different subnets. We allocate two of the five servers as clients, and the other three act as servers. The load balancer runs on the server subnet, receiving and forwarding requests from the same NIC, i.e., router-on-a-stick. Figure~\ref{fig:eval-topo} shows the path of a request to one of the backend servers. \texttt{Nginx} is configured as the server software with static file serving of varied file sizes. \texttt{wrk} and \texttt{wrk2} are used with customized Lua script as the client software. 
\begin{figure}[htbp]
\vspace{-0.5cm}
\centering
\includegraphics[width=0.35\textwidth, keepaspectratio]{evals/eval_topo-cropped.pdf}
\vspace{-0.2cm}
\caption{A request from the client to the backend server}
\label{fig:eval-topo}
\vspace{-0.3cm}
\end{figure}


There are multiple widely adopted L7 load balancers on the market, including Envoy~\cite{envoy}, Nginx~\cite{nginx}, HAProxy~\cite{haproxy}, etc. We choose Nginx as our baseline since it is widely adopted and high-performance compared with others~\cite{dropboxnginx}.

%\begin{itemize}
%    \item We use 2 client 2 server
%    \item Config L4 routing on the switch side
%    \item We use Nginx as the server, wrk as the client
%\end{itemize}
%
%\begin{itemize}
%    \item Server and client config: CPU, RAM
%    \item Network downgrade to 50Gbps
%\end{itemize}


%The evaluation answers the following questions:
%\begin{itemize}
%    \item Just use general purpose processing on the same hardware, whether our design outperform existing %software 
%    \item Whether \sys on SmartNIC has the same even better throughput compared with commodity server despite ARM %is slow
%    \item Whether our performance keeps up with increasing number of connections
%    \item Whether our system scales well with increasing number of cores
%    \item Whether offloading provides significant throughput gain
%    \item How does the performance of \sys with real hybrid workload?
%\end{itemize}

Our evaluation answers the following questions:
\squishlist
    \item Will \sys outperform the widely-used L7 load balancer Nginx? We evaluate the throughput of \sys on various response sizes on both LiquidIO3 and BlueField-2. We also compare the flow completion times of \sys and Nginx.
    \item Will \sys achieve performance gains by offloading packet processing onto the hardware engines, thus relieving the generic SmartNIC cores? We experimentally set 1M as the offload threshold to evaluate the performance.
    \item Will \sys achieve good scalability as we increase the number of processing cores on the SmartNIC? We then evaluate the throughput while varying the number of cores.
    \item Will \sys perform well with a realistic workload comprising of mixed flow sizes? We play a trace with the mixed sizes and compare the performance of \sys and Nginx.
\squishend

\subsection{Microbenchmark}

%\begin{enumerate}
%    \item [Fin] line gragh: x: response size y: NginxLIO3, LIO3, Nginxx86 (rps, gbps), all core
%    \item line gragh: x: response size y: NginxLIO3, LIO3, Nginxx86 (rps, gbps), Single core
%    \item [Fin] line gragh: x: response size y: BluefieldNginx, Bluefield, Nginxx86 (rps, gbps), all core
%    \item line gragh: x: response size y: BluefieldNginx, Bluefield, Nginxx86 (rps, gbps), Single core
%    \item bar gragh: x: number of cores 1, 2, 4, 8, 16 y: rps (10k), LIO3, Nginxx86, LIO3x86, LIO3Nginx
%    \item bar gragh: x: number of cores 1, 2, 4, 8 y: rps (10k) Bluefield, Nginxx86, BluefieldNginx
%    \item bar graph: Bluefield offload, Bluefield no offload, Bluefield Nginx compare, 10M, 100M, 6 point
%\end{enumerate}

%Arvind notes on evaluation:
%\begin{itemize}
    %\item Split off a version of Fig 6 for the motivation section.  This will include throughput per core for x86 running Nginx and LIO3 running Nginx.  Makes the point that LIO3 cores are not very fast.
    %\item Looks like the larger transfers aren't super interesting.  Maybe stop at 10M and introduce a couple of smaller transfer sizes.  
    %\item Plot rps in log scale on the y axis?
    %\item 10M single core performance on BF is not quite right I think
    %\item BF has a scalability loss at 7 cores for the real workload.  Might need to debug this
%\end{itemize}

We generate a list of static files with various file sizes to evaluate the behavior of \sys compared against Nginx. We use \texttt{wrk} to measure the metric of requests per second data, and we multiply it by the file size to get the goodput measurement. Since the same port on these devices will receive data from both the requests of the clients and also receive the responses from the backend servers, the theoretical upper limit for the load balancer's goodput is lower than the line rate. 

Since the LiqudIO3 device can only support 50Gbps link speed, we also cap the X86 baseline at 50Gbps for a fair comparison for all the experiments running on LiquidIO3.
\begin{figure}[htbp]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/lio3_fixed_gbps.pdf}
\caption{Lio3 Fixed response size throughput (Gbps)}
\label{fig:lio3fixedgbps}
\vspace{-0.1cm}
\end{figure}

Figure~\ref{fig:lio3fixedgbps} shows the throughput of the different configurations on LiquidIO3 50G NIC with 24 arm cores. Nginx on the Arm cores of the SmartNIC (bar "LIO3 Nginx") has a low throughput. The throughput plateaus at around 5Gbps even with 24 cores. \sys can easily reach the full NIC bandwidth with 10K response size. However, Nginx running on a x86 server needs 32 beefy to achieve the comparable performance. 


Next, we evaluate the throughput on off-path BlueField-2 SmartNICs. The BlueField-2 device is equipped with 2x100G ports. We enabled the two ports together to further stress the processing power on the Arm cores. For the baseline, we use both 100G ports on a ConnectX5 NIC to make the link speed the same. However, although there are 2x100G ports on ConnectX 5, due to the bottleneck of PCIe 3.0, only about 120Gbps can be achieved. As shown in Figure~\ref{fig:bffixedgbps}, a SmartNIC with only 8 NIC cores can achieve line rate for large message sizes, and for small packets, \sys achieves comparable performance with Nginx running on x86. 
\begin{figure}[htbp]
\centering
         \includegraphics[width=0.49\textwidth, keepaspectratio]{evals/200GBF_fixed_gbps.pdf}
\vspace{-0.5cm}
\caption{Bluefield Fixed response size throughput (Gbps)}
\label{fig:bffixedgbps}
\end{figure}
Bluefield has weak Arm cores, and it performs poorly for Nginx as expected. There is a clear increase in throughput from 1M to 4M because \sys offloads the packet processing into the hardware engine for response sizes larger than 1M. Other than the first few packets, all of the remaining packets in that flow are purely processed by the hardware packet processing engine. This can mitigate the head of line blocking problem caused by limited processing power and also relieves the CPU resources for small or future responses. 

To clearly show the single-core processing capability for \sys, we further evaluate the throughput on just one core by varying the response size. As shown in Figure~\ref{fig:singlecorelio3gbps}, \sys on LIO3 performs much better than Nginx, even though Nginx runs on a more powerful x86 core. Figure~\ref{fig:singlecorebfgbps} clearly shows it is the same case that the single-core performance of \sys on BlueField-2 outperforms Nginx on x86. For response sizes of 16M, \sys achieves 16x throughput compared with Nginx x86 with the help of the hardware flow processing engine. On LiquidIO3, which does not have a hardware flow processing engine, the throughput of \sys is 4.5x better compared with x86 Nginx.
\begin{figure}[htbp]
\centering
\vspace{-0.2cm}
\includegraphics[width=0.4\textwidth, keepaspectratio]{evals/singlecore_lio3_gbps.pdf}
\vspace{-3mm}
\caption{Single-core throughput of LiquidIO3 (Gbps)}
\vspace{-2mm}
\label{fig:singlecorelio3gbps}
\end{figure}
\begin{figure}[htbp]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/singlecore_200GBF_fixed_gbps.pdf}
\caption{Single core throughput of Bluefield (Gbps)}
\vspace{-0.3cm}
\label{fig:singlecorebfgbps}
\end{figure}

To show the scalability behavior, we measure the throughput by increasing the number of cores. Figure ~\ref{fig:bfdiffcore} shows that even with the lock-free data structures in \sys, it is hard to reach the full NIC bandwidth with the Arm cores for small response sizes. While offloading the processing into a hardware engine after 1M, it can easily reach 200G full NIC bandwidth. Figure~\ref{fig:lio3diffcore} depicts the scalability data for LIO3, where we see linear increases in throughput till line rate is achieved, except for the 1KB flow case.
%\begin{figure}[htbp]
%\centering
%         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/lio3_fixed_rps.pdf}
%\caption{Lio3 Fixed response size throughput (rps)}
%\label{fig:lio3fixedrps}
%\end{figure}

%\begin{figure}[htbp]
%\centering
%         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/bluefield_fixed_rps.pdf}
%\caption{Bluefield Fixed response size throughput (rbps)}
%\label{fig:bffixedrps}
%\end{figure}

\begin{figure}[htbp]
\centering
\vspace{-0.3cm}
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/200GBF_scale.pdf}
\vspace{-0.3cm}
\caption{Bluefield with a different number of cores (Gbps)}
\label{fig:bfdiffcore}
\end{figure}
\begin{figure}[htbp]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/lio3_scale.pdf}
\vspace{-0.2cm}
\caption{LIO3 with different number of cores (Gbps)}
\label{fig:lio3diffcore}
\end{figure}

We next study the performance of our lightweight networking stack in terms of the flow completion times. We use \texttt{wrk2} with a target throughput of 50\% peak throughput we measured in the previous experiments and recorded the flow completion times. 
\cxyzhao{Is this BF2 LACONIC?}
Figure~\ref{fig:latencyrespsize} shows an overview of the flow completion time with single core. Despite our design running on Bluefield with a higher target throughput, Laconic's flow completion times are comparable to that of the Nginx x86.
\begin{figure}[h]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/latency_respsize.pdf}
\caption{Flow completion time of different resposne size: single core (match Figure~\ref{fig:singlecorebfgbps})}
\vspace{-0.1cm}
\label{fig:latencyrespsize}
\end{figure}

\begin{figure}[h]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/latency_respsize_allcore.pdf}
\caption{Flow completion time of different resposne size: all core (match Figure~\ref{fig:bffixedgbps})}
\vspace{-0.1cm}
\label{fig:latencyrespsize_allcore}
\end{figure}

\begin{figure}[h]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/latency_bf_core.pdf}
\caption{Flow completion time of different cores on Bluefield (match Figure~\ref{fig:bfdiffcore})}
\vspace{-0.1cm}
\label{fig:latency_corenum}
\end{figure}


We further zoom in to a specific response size to plot the cumulative distribution function (CDF) in Figure~\ref{fig:latency1Kcdf}. We compare \sys and Nginx on BlueField-2 and show that we achieve lower flow completion times when compared to Nginx running on the Arm cores or the x86 cores.
\begin{figure}[h]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/latency_1K_cdf.pdf}
\caption{CDF for flow completion time on different platforms with 1K response size}
\label{fig:latency1Kcdf}
\end{figure}

%\begin{figure}[htbp]
%\centering
%         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/offload.pdf}
%\caption{Bluefield with offload and without offload (Gbps)}
%\label{fig:bfoffload}
%\end{figure}
\subsection{Real-world workload}
To evaluate the performance of \sys\ under a real-world workload, we adopt the data from the CONGA work on datacenter traffic load balancing~\cite{conga}. We extract the flow size distribution from their enterprise workload. We generate a list of files corresponding to the flow sizes on the backend server. On the client-side, we use a customized Lua script for \texttt{wrk} to generate the request according to the distribution. With the mixed workload, we use two metrics to evaluate the throughput: a) Goodput measured in gigabits per second; b) Requests per second. With the varying flow sizes, higher requests per second might not represent or lead to higher network throughput, so we use these two metrics to fully evaluate the performance.
\begin{figure}[htbp]
\vspace{-0.5cm}
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/real_gbps_lio3.pdf}
         %\vspace{0.4cm}
\caption{Enterprise workload throughput for LiquidIO3 (Gbps)}
\label{fig:realgbps-lio3}
\end{figure}

\begin{figure}[htbp]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/real_rps_lio3.pdf}
         \vspace{-0.3cm}
\caption{Enterprise workload throughput for LiquidIO3 (rps)}
\label{fig:realrps-lio3}
\end{figure}

LIO3 has 24 Arm cores, so we perform the tests on LIO3 with up to 24 cores. From Figure~\ref{fig:realgbps-lio3} and Figure~\ref{fig:realrps-lio3}, we observe that Nginx on LIOs runs at a very low throughput (5.21Gbps and 24,374 requests per second). Nginx on x86 linearly increases the performance; however, it needs more than 16 cores for just 50G bandwidth. In contrast, \sys only needs up to two Arm cores to match the 50G NIC bandwidth.  

%Figure~\ref{fig:realgbps-lio3} and figure~\ref{fig:realrps-lio3} show on LiquidIO3, with fewer number of cores, we can outperform the throughput of x86 on both the request per second and the Gbps metrics. We use two metric since the flow size varies and higher requests per second does not necessary lead to higher networking throughput if the large response is suffered from starvation.
\begin{figure}[htbp]
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/real_gbps_bf.pdf}
\caption{Enterprise workload throughput for Bluefield (Gbps)}
\label{fig:realgbps-bf}
\end{figure}
\begin{figure}[h]
\vspace{-0.2cm}
\centering
         \includegraphics[width=0.4\textwidth, keepaspectratio]{evals/real_rps_bf.pdf}
\caption{Enterprise workload throughput for Bluefield (rps)}
\label{fig:realrps-bf}
\end{figure}

We further demonstrate the throughput of \sys with the real-world workload on BlueField-2, which only has 8 Arm cores. \cxyzhao{more results} In Figure ~\ref{fig:realgbps-bf} and Figure~\ref{fig:realrps-bf}, we observe the same trend as LIO3. \sys can achieve 20x throughput with a single core compared to Nginx running on BlueField-2. It has higher performance with a fewer number of cores up to 75Gbps; however, Nginx needs more than 16 cores to achieve a similar speed.
%Figure ~\ref{fig:realrps-bf} and figure~\ref{fig:realgbps-bf} demonstrate the performance of of \sys on Bluefield. With a limited number of cores available on Bluefield, \sys achieve 20x throughput for single core performance compared to Nginx running on Bluefield.

